Rethinking Word-Level Auto-Completion in Computer-Aided Translation

Word-Level Auto-Completion (WLAC) plays a crucial role in Computer-Assisted Translation. It aims at providing word-level auto-completion suggestions for human translators. While previous studies have primarily focused on designing complex model architectures, this paper takes a different perspective by rethinking the fundamental question: what kind of words are good auto-completions? We introduce a measurable criterion to answer this question and discover that existing WLAC models often fail to meet this criterion. Building upon this observation, we propose an effective approach to enhance WLAC performance by promoting adherence to the criterion. Notably, the proposed approach is general and can be applied to various encoder-based architectures. Through extensive experiments, we demonstrate that our approach outperforms the top-performing system submitted to the WLAC shared tasks in WMT2022, while utilizing significantly smaller model sizes.

==> 1-intro-v1.tex <==
In recent years, the field of machine translation has witnessed a remarkable performance surge, driven by the abundance of multilingual data and the emergence of larger models. With the increasing reliance on multilingual data, the efficiency of data labeling becomes increasingly crucial. Consequently,  the attention of researchers has increasingly been drawn to leveraging the advancements in automatic machine translation to enhance the translation efficiency of human translators.

Interactive machine translation (IMT) is a subfield of computer-aided translation (CAT) that aims to assist human translators by predicting their input text. The word-level auto-completion (WLAC) task is the core function of IMT, which involves predicting the word being typed by the translator given the translation context. Figure \ref{example} illustrates an example of such auto-completion. Effective auto-suggestions have the potential to reduce keystrokes by at least $60\%$ during the translation process\citep{input_method}. A user survey indicates that $90.2\%$ of participants find the word-level auto-suggestion feature helpful\citep{survey}. Therefore, the performance of the WLAC task plays an important role in the effectiveness of IMT.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{emnlp2023-latex/images/example.png}
    \caption{An example of word-level auto completion. Assume the human translator is translating a Chinese sentence to English. The corresponding meaning of Chinese words are marked in brackets for better understanding.}
    \label{example}
\end{figure}

The general word-level auto-complete (WLAC) task was initially formulated by \citet{li-etal-2021-gwlan}, who also introduced a publicly available benchmark for evaluating this task. One of the main challenges in WLAC lies in handling the discontinuity of the translation context. In real translation scenarios, translators often encounter situations where they need to add or modify words within a sentence. During most of the translation process, the model can only access to limited and incomplete context. 



To address this challenge, \citet{li-etal-2021-gwlan} proposed a model that utilizes two encoders to process the source sentence and translation context, predicting the target word using a mask-prediction approach. However, their approach does not leverage the machine translation task.
Recently, \citet{yang2022hw} proposed a novel approach where a machine translation model is pre-trained and then fine-tuned specifically for the WLAC task. Their findings demonstrate significant performance improvements by incorporating the machine translation task into WLAC. Nevertheless, it is important to note that WLAC, which focuses on word prediction, differs from the translation task, so directly finetuning a translation model for WLAC may result in the model forgetting its translation-specific knowledge. Hence, there is a need to explore more effective methods for leveraging the translation task within the context of WLAC.



As illustrated in Figure \ref{example}, we think a golden predicting procedure can be: firstly generate a complete translation based on the existing context (e.g. "\textit{The answer to}"), then select the best word from the translation according to the input position and typed sequence (e.g. "\textit{an}"). Based on this insight, we propose to introduce machine translation as an auxiliary task and jointly train the translation task and WLAC task. We use an encoder to encode all the input and make the word prediction, and stack a decoder on the encoder to conduct translation task. The decoder explicitly perform translation planning during training and introduce additional translation signal to guide the WLAC prediction. Once the training is done, the translation knowledge has been injected into the model and we no longer need the decoder during inference, which can further reduce the model size. Our experiment result shows that with joint training, the word-level model can outperform the state of the art BPE-level model, combine the joint training framework with BPE-level model can even push the performance further. We also conduct detailed analysis on the model prediction and the findings suggest that our approach can effectively leverage machine translation task to improve WLAC task.

To conclude, our contributions are listed as follows:
\begin{itemize}
    \item We propose a general joint training framework for introducing machine translation task into the WLAC task.
    \item Experiment results show that the proposed method can outperform SOTA models by a large margin while our model is much smaller and faster.
    \item We extensively analyze the model prediction and provide insights about how this framework work and how to further improve the model.
\end{itemize}

